MMHQA-ICL: Multimodal In-context Learning for Hybrid Question Answering over Text, Tables and Images

In the real world, knowledge often exists in a multimodal and heterogeneous form. Addressing the task of question answering with hybrid data types, including text, tables, and images, is a challenging task (MMHQA). Recently, with the rise of large language models (LLM), in-context learning (ICL) has become the most popular way to solve QA problems. We propose MMHQA-ICL framework for addressing this problems, which includes stronger heterogeneous data retriever and an image caption module. Most importantly, we propose a Type-specific In-context Learning Strategy for MMHQA, enabling LLMs to leverage their powerful performance in this task. We are the first to use end-to-end LLM prompting method for this task. Experimental results demonstrate that our framework outperforms all baselines and methods trained on the full dataset, achieving state-of-the-art results under the few-shot setting on the MultimodalQA dataset.

==> tables/ar_poster.tex <==
\begin{table*}
\centering
\scalebox{0.74}{
\begin{tabular}{lccccccccccc}
\toprule
Dataset & Input & \#Inputs & Evidence & Verdict & Sources & Lang \\
\midrule
FEVER~\citep{Thorne2018FEVERAL} & State & 185,445  & Text & 3Class & Wiki & En \\
HOVER~\citep{jiang2020hover} & State & 26,171  & Text & 2Class & Wiki & En  \\
% WikiFactCheck~\citep{SatheALPP20} & State & 124,821  & Text & 2Class & Wiki & En  \\
% Symmetric \citep{Schuster2019TowardsDF} & State & 956  & Text & 3 & Wikipedia & En \\
% FM2 \citep{foolme2021} & State & 12,968  & Text & 3 & Wikipedia & En \\
VitaminC~\citep{vitaminc2021} & State & 488,904  & Text & 3Class & Wiki & En \\
TabFact~\citep{Chen2020TabFactAL} & State & 92,283  & Table & 2Class & Wiki & En \\
InfoTabs~\citep{Gupta2020INFOTABSIO} & State & 23,738  & Table & 3Class & Wiki & En \\
Sem-Tab-Fact~\citep{wang2021semeval} & State & 5,715  & Table & 3Class & Wiki & En \\
FEVEROUS~\citep{Aly2021FEVEROUSFE} & State & 87,026  & Text/Table & 3Class & Wiki & En \\
% ANT~\citep{Khouja2020StancePA} & State & 4,547  & \xmark & 3Class & News & Ar \\
% DanFEVER~\citep{NorregaardD21} & State & 6,407  & Text & 3 Classes & Wiki & Da \\
\bottomrule
\end{tabular}}
\vspace{-0.5em}
\caption{Summary of factual verification datasets with artificial inputs. Google denotes Google Relation Extraction Corpora, and WSDM means the WSDM Cup 2017 Triple Scoring challenge.}
\label{tab:artificial}
\vspace{-1em}
\end{table*}

==> tables/artificial.tex <==
\begin{table*}
\centering
\scalebox{0.74}{
\begin{tabular}{lccccccccccc}
\toprule
Dataset & Input & \#Inputs & Evidence & Verdict & Sources & Lang \\
\midrule
KLinker~\citep{Ciampaglia2015ComputationalFC} & Triple & 10,000  & KG & 2 Classes & Google/Wiki & En \\
PredPath~\citep{ShiW16} & Triple & 3,559  & KG & 2 Classes & Google/Wiki & En \\
% KStream~\citep{Shiralkar2017FindingSI} & Triple & 18,431  & KG & 2 Classes & Google/Wiki/WSDM & En \\
KStream~\citep{Shiralkar2017FindingSI} & Triple & 18,431  & KG & 2 Classes & Google/Wiki & En \\
UFC~\citep{kim-choi-2020-unsupervised} & Triple & 1,759  & KG & 2 Classes & Wiki & En \\
\midrule
LieDetect~\citep{mihalcea2009lie} & Passage & 600  & \xmark & 2 Classes & News & En \\
FakeNewsAMT~\citep{PrezRosas2018AutomaticDO} & Passage & 680  & \xmark & 2 Classes & News & En \\
\midrule
FEVER~\citep{Thorne2018FEVERAL} & Statement & 185,445  & Text & 3 Classes & Wiki & En \\
HOVER~\citep{jiang2020hover} & Statement & 26,171  & Text & 2 Classes & Wiki & En  \\
WikiFactCheck~\citep{SatheALPP20} & Statement & 124,821  & Text & 2 Classes & Wiki & En  \\
% Symmetric \citep{Schuster2019TowardsDF} & Statement & 956  & Text & 3 & Wikipedia & En \\
% FM2 \citep{foolme2021} & Statement & 12,968  & Text & 3 & Wikipedia & En \\
VitaminC~\citep{vitaminc2021} & Statement & 488,904  & Text & 3 Classes & Wiki & En \\
TabFact~\citep{Chen2020TabFactAL} & Statement & 92,283  & Table & 2 Classes & Wiki & En \\
InfoTabs~\citep{Gupta2020INFOTABSIO} & Statement & 23,738  & Table & 3 Classes & Wiki & En \\
Sem-Tab-Fact~\citep{wang2021semeval} & Statement & 5,715  & Table & 3 Classes & Wiki & En \\
FEVEROUS~\citep{Aly2021FEVEROUSFE} & Statement & 87,026  & Text/Table & 3 Classes & Wiki & En \\
ANT~\citep{Khouja2020StancePA} & Statement & 4,547  & \xmark & 3 Classes & News & Ar \\
DanFEVER~\citep{NorregaardD21} & Statement & 6,407  & Text & 3 Classes & Wiki & Da \\
\bottomrule
\end{tabular}}
\vspace{-0.5em}
\caption{Summary of factual verification datasets with artificial inputs. Google denotes Google Relation Extraction Corpora, and WSDM means the WSDM Cup 2017 Triple Scoring challenge. (Data collected by \cite{guo-etal-2022-survey})}
\label{tab:artificial}
\vspace{-1em}
\end{table*}

==> tables/de_poster.tex <==
\begin{table*}
\centering
\scalebox{0.74}{
\begin{tabular}{lcccccc}
\toprule
Dataset & Type & Input & \#Inputs & Evidence & Verdict & Lang \\
\midrule
CredBank~\citep{MitraG15} & Worthy & Aggregate & 1,049  & Meta & 5 Classes  & En \\
Weibo~\citep{Ma2016DetectingRF} & Worthy & Aggregate & 5,656  & Meta & 2 Classes  & En/Ch  \\
% Weibo20 \citep{zhang2021mining} & Aggregate & 6,362 & 2 & Meta & Weibo & Ch \\
PHEME~\citep{zubiaga2016analysing} & Worthy & Individual & 330  & Text/Meta & 3 Classes  & En/De \\
% RumourEval \citep{Derczynski2017SemEval2017T8} & Worthy & Individual & 325  & Text/Meta & 3 & Twitter & En \\
RumourEval19~\citep{GorrellABDKLZ19} & Worthy & Individual & 446 & Text/Meta & 3 Classes  & En \\
DAST~\citep{Lillie2019JointRS} & Worthy & Individual & 220  & Text/Meta & 3 Classes  & Da \\
Suspicious~\citep{Volkova2017SeparatingFF} & Worthy & Individual & 131,584  & \xmark & 2/5 Classes  & En \\
CheckThat20-T1~\citep{BarrnCedeo2020OverviewOC} & Worthy & Individual & 8,812  & \xmark & Ranking  & En/Ar \\
CheckThat21-T1A~\citep{NakovMEBMSAHHBN21} & Worthy & Individual & 17,282  & \xmark & 2 Classes & Many \\
% FauxBuster \citep{Zhang2018FauxBusterAC} & Worthy & Individual$^{\dagger}$ & 917  & Meta  & 2 & Twitter/Reddit & En \\
% COVIDLIES \citep{Hossain2020COVIDLiesDC} & Worthy & Individual & 6,761 & Misconception & 3 & Twitter & En \\
% \midrule
Debate~\citep{hassan2015detecting} & Worthy & Statement & 1,571  & \xmark & 3 Classes  & En \\
ClaimRank~\citep{Gencheva2017ACA} & Worthy & Statement & 5,415  & \xmark & Ranking  & En \\
CheckThat18-T1~\citep{Atanasova2018OverviewOT} & Worthy & Statement & 16,200  & \xmark & Ranking  & En/Ar \\
% CheckThat19-T1 \citep{CheckThat2019} & Claim & 23,500 & ranking & \xmark & Transcript & En \\
% CheckThat20-T5 \citep{BarrnCedeo2020OverviewOC} & Claim & 64,290 & ranking & \xmark & Transcript & En \\
% CheckThat21-T1B \citep{clef2021} & Claim & 84,290 & ranking & \xmark & Transcript & En \\
\midrule
%\midrule
CitationReason~\citep{redi2019}  & Checkable & Statement & 4,000  & Meta & 13 Classes  & En \\
PolitiTV~\citep{konstantinovskiy2018towards} & Checkable & Statement & 6,304  & \xmark & 7 Classes  & En \\
%SemEval19-TA\citep{Mihaylova2019SemEval2019T8} & Checkable & Question & 2,310 & Meta  & 3 & Forum & En \\
\bottomrule
\end{tabular}}
\vspace{-0.5em}
\caption{Summary of claim detection datasets. Input can be a set of posts (aggregate) or an individual post from social media, or a statement. Evidence include text and metadata. Verdict can be a multi-class label or a rank list.}
% En, De, Ch, Ar, and Da indicate English, German, Chinese, Arabic, and Danish, respectively.}
% \citet{NakovMEBMSAHHBN21} offered datasets in Arabic, Bulgarian, English, and Spanish.}
\label{tab:detection}
\vspace{-1em}
\end{table*}

==> tables/detection.tex <==
\begin{table*}
\centering
\scalebox{0.74}{
\begin{tabular}{lccccccc}
\toprule
Dataset & Type & Input & \#Inputs & Evidence & Verdict & Sources & Lang \\
\midrule
CredBank~\citep{MitraG15} & Worthy & Aggregate & 1,049  & Meta & 5 Classes & Twitter & En \\
Weibo~\citep{Ma2016DetectingRF} & Worthy & Aggregate & 5,656  & Meta & 2 Classes &  Twitter/Weibo & En/Ch  \\
% Weibo20 \citep{zhang2021mining} & Aggregate & 6,362 & 2 & Meta & Weibo & Ch \\
PHEME~\citep{zubiaga2016analysing} & Worthy & Individual & 330  & Text/Meta & 3 Classes & Twitter & En/De \\
% RumourEval \citep{Derczynski2017SemEval2017T8} & Worthy & Individual & 325  & Text/Meta & 3 & Twitter & En \\
RumourEval19~\citep{GorrellABDKLZ19} & Worthy & Individual & 446 & Text/Meta & 3 Classes & Twitter/Reddit & En \\
DAST~\citep{Lillie2019JointRS} & Worthy & Individual & 220  & Text/Meta & 3 Classes & Reddit & Da \\
Suspicious~\citep{Volkova2017SeparatingFF} & Worthy & Individual & 131,584  & \xmark & 2/5 Classes & Twitter & En \\
CheckThat20-T1~\citep{BarrnCedeo2020OverviewOC} & Worthy & Individual & 8,812  & \xmark & Ranking & Twitter & En/Ar \\
CheckThat21-T1A~\citep{NakovMEBMSAHHBN21} & Worthy & Individual & 17,282  & \xmark & 2 Classes & Twitter & Many \\
% FauxBuster \citep{Zhang2018FauxBusterAC} & Worthy & Individual$^{\dagger}$ & 917  & Meta  & 2 & Twitter/Reddit & En \\
% COVIDLIES \citep{Hossain2020COVIDLiesDC} & Worthy & Individual & 6,761 & Misconception & 3 & Twitter & En \\
% \midrule
Debate~\citep{hassan2015detecting} & Worthy & Statement & 1,571  & \xmark & 3 Classes & Transcript & En \\
ClaimRank~\citep{Gencheva2017ACA} & Worthy & Statement & 5,415  & \xmark & Ranking & Transcript & En \\
CheckThat18-T1~\citep{Atanasova2018OverviewOT} & Worthy & Statement & 16,200  & \xmark & Ranking & Transcript & En/Ar \\
% CheckThat19-T1 \citep{CheckThat2019} & Claim & 23,500 & ranking & \xmark & Transcript & En \\
% CheckThat20-T5 \citep{BarrnCedeo2020OverviewOC} & Claim & 64,290 & ranking & \xmark & Transcript & En \\
% CheckThat21-T1B \citep{clef2021} & Claim & 84,290 & ranking & \xmark & Transcript & En \\
\midrule
%\midrule
CitationReason~\citep{redi2019}  & Checkable & Statement & 4,000  & Meta & 13 Classes & Wikipedia & En \\
PolitiTV~\citep{konstantinovskiy2018towards} & Checkable & Statement & 6,304  & \xmark & 7 Classes & Transcript & En \\
%SemEval19-TA\citep{Mihaylova2019SemEval2019T8} & Checkable & Question & 2,310 & Meta  & 3 & Forum & En \\
\bottomrule
\end{tabular}}
\vspace{-0.5em}
\caption{Summary of claim detection datasets. Input can be a set of posts (aggregate) or an individual post from social media, or a statement. Evidence include text and metadata. Verdict can be a multi-class label or a rank list. (Data collected by \cite{guo-etal-2022-survey})}
% En, De, Ch, Ar, and Da indicate English, German, Chinese, Arabic, and Danish, respectively.}
% \citet{NakovMEBMSAHHBN21} offered datasets in Arabic, Bulgarian, English, and Spanish.}
\label{tab:detection}
\vspace{-1em}
\end{table*}

==> tables/na_poster.tex <==
\begin{table*}
\centering
\scalebox{0.74}{
\begin{tabular}{lccccccccccc}
\toprule
Dataset & Input & \#Inputs & Evidence & Verdict & Sources & Lang \\
\midrule

Politifact~\citep{Vlachos2014FactCT}  & State  & 106  & Text/Meta & 5Class & Factcheck & En \\
% NewsTrust \citep{Mukherjee2015LeveragingJI}  & State  & 106 & 5 & Text  & Factcheck & En \\
Emergent~\citep{Ferreira2016EmergentAN} & State & 300  & Text & 3Class & Emergent & En \\
% CreditAssess~\citep{Popat2016CredibilityAO} & State & 5,013 & Text & 2 Classes & Factcheck/Wiki & En \\
PunditFact~\citep{Rashkin2017TruthOV} & State  & 4,361  & \xmark & 2/6Class & Factcheck & En \\
Liar~\citep{Wang2017LiarLP} & State  & 12,836  & Meta & 6Class & Factcheck & En \\
% Liar-Plus \citep{Alhindi2018WhereIY} & State & 12,836 & 6 & Text/Meta & Factcheck & En \\
% CheckThat19-T2 \citep{HasanainSEBN19} & State &  69  & Text & 2 & News & En\\
Snopes~\citep{Hanselowski2019ARA} & State & 6,422  & Text & 3Class & Factcheck & En \\
MultiFC~\citep{Augenstein2019MultiFCAR} & State & 36,534  & Text/Meta & 2-27Class &  Factcheck & En \\
% Climate-FEVER~\citep{diggelmann2020} & State & 1,535 & Text  & 4 Classes & Climate & En \\
SciFact~\citep{Wadden2020FactOF} & State & 1,409  & Text & 3Class & Science & En \\
Health~\citep{kotonya2020explainable} & State & 11,832  & Text & 4Class & Factcheck & En\\

X-Fact~\citep{gupta-srikumar-2021-x} & State & 31,189  & Text & 7Class & Factcheck & Many\\
\midrule
FEVER~\citep{Thorne2018FEVERAL} & State & 185,445  & Text & 3Class & Wiki & En \\
HOVER~\citep{jiang2020hover} & State & 26,171  & Text & 2Class & Wiki & En  \\
% WikiFactCheck~\citep{SatheALPP20} & State & 124,821  & Text & 2Class & Wiki & En  \\
% Symmetric \citep{Schuster2019TowardsDF} & State & 956  & Text & 3 & Wikipedia & En \\
% FM2 \citep{foolme2021} & State & 12,968  & Text & 3 & Wikipedia & En \\
VitaminC~\citep{vitaminc2021} & State & 488,904  & Text & 3Class & Wiki & En \\
TabFact~\citep{Chen2020TabFactAL} & State & 92,283  & Table & 2Class & Wiki & En \\
InfoTabs~\citep{Gupta2020INFOTABSIO} & State & 23,738  & Table & 3Class & Wiki & En \\
Sem-Tab-Fact~\citep{wang2021semeval} & State & 5,715  & Table & 3Class & Wiki & En \\
FEVEROUS~\citep{Aly2021FEVEROUSFE} & State & 87,026  & Text/Table & 3Class & Wiki & En \\
% \midrule
% % SemEval19-TB \citep{Mihaylova2019SemEval2019T8} & Answer & 917  & Meta & 3 & Forum & En \\
% AnswerFact~\citep{Zhang2020AnswerFactFC} & Answer & 60,864 & Text & 5 Classes & Amazon & En \\
% \midrule
% % Hoax \citep{TacchiniBVMA17} & Article & 15,500  & Meta & 2 Classes & Facebook & En \\
% NELA~\citep{HorneKA18} & Article & 136,000  & \xmark & 2 Classes & News & En \\
% BuzzfeedNews \citep{Potthast2018ASI} & Article & 1,627 & Meta & 4 Classes & Facebook & En \\
% BuzzFace~\citep{SantiaW18} & Article & 2,263 & Meta & 4 Classes & Facebook & En \\
% % NELA18 \citep{Nrregaard2019NELAGT2018AL} & Article & 713,000 & 2 & \xmark & News & En \\
% % NELA19 \citep{gruppi2020nela} & Article & 1.12M & 2 & \xmark & News & En \\
% FA-KES~\citep{SalemFEJF19} & Article & 804 & \xmark & 2 Classes & VDC & En \\
% FakeNewsNet \citep{Shu2018FakeNewsNetAD} & Article & 23,196  & Meta & 2 Classes & Factcheck & En \\
% %FakeHealth \citep{DaiSW20} & Article & 2,296  & Meta & 2 Classes & Health & En \\
% FakeCovid~\citep{shahifakecovid} & Article & 5,182  & \xmark & 2 Classes & Factcheck & Many \\
% \midrule
% Fauxtography \citep{Zlatkova2019FactCheckingMF} & State/Image & 1,233  & Meta & 2 & Factcheck/News & En \\
% Fakeddit \citep{Nakamura2020rFakedditAN} & State/Image & 1.06M  & Meta & 2,3,6 & Reddit & En \\
\bottomrule
\end{tabular}}
\vspace{-0.5em}
\caption{Summary of factual verification datasets with natural inputs. KG denotes knowledge graphs. ChectThat18 has been extended later~\citep{HasanainSEBN19,BarrnCedeo2020OverviewOC,NakovMEBMSAHHBN21}. NELA has been updated by adding more data from more diverse sources~\citep{NorregaardHA19,gruppi2020,gruppi2021}
}
\label{tab:natural}
\vspace{-1em}
\end{table*}

==> tables/natural.tex <==
\begin{table*}
\centering
\scalebox{0.74}{
\begin{tabular}{lccccccccccc}
\toprule
Dataset & Input & \#Inputs & Evidence & Verdict & Sources & Lang \\
\midrule
CrimeVeri~\citep{bachenko-etal-2008-verification} & Statement & 275 & \xmark & 2 Classes & Crime & En \\
Politifact~\citep{Vlachos2014FactCT}  & Statement  & 106  & Text/Meta & 5 Classes & Fact Check & En \\
StatsProperties~\citep{vlachos-riedel-2015-identification} & Statement & 7,092  & KG & Numeric & Internet & En \\
% NewsTrust \citep{Mukherjee2015LeveragingJI}  & Statement  & 106 & 5 & Text  & Fact Check & En \\
Emergent~\citep{Ferreira2016EmergentAN} & Statement & 300  & Text & 3 Classes & Emergent & En \\
CreditAssess~\citep{Popat2016CredibilityAO} & Statement & 5,013 & Text & 2 Classes & Fact Check/Wiki & En \\
PunditFact~\citep{Rashkin2017TruthOV} & Statement  & 4,361  & \xmark & 2/6 Classes & Fact Check & En \\
Liar~\citep{Wang2017LiarLP} & Statement  & 12,836  & Meta & 6 Classes & Fact Check & En \\
% Liar-Plus \citep{Alhindi2018WhereIY} & Statement & 12,836 & 6 & Text/Meta & Fact Check & En \\
Verify~\citep{Baly2018IntegratingSD} & Statement & 422  & Text & 2 Classes & Fact Check & Ar/En \\
CheckThat18-T2 \citep{Barron-CedenoES18} & Statement & 150  & \xmark & 3 Classes & Transcript & En \\
% CheckThat19-T2 \citep{HasanainSEBN19} & Statement &  69  & Text & 2 & News & En\\
Snopes~\citep{Hanselowski2019ARA} & Statement & 6,422  & Text & 3 Classes & Fact Check & En \\
MultiFC~\citep{Augenstein2019MultiFCAR} & Statement & 36,534  & Text/Meta & 2-27 Classes &  Fact Check & En \\
Climate-FEVER~\citep{diggelmann2020} & Statement & 1,535 & Text  & 4 Classes & Climate & En \\
SciFact~\citep{Wadden2020FactOF} & Statement & 1,409  & Text & 3 Classes & Science & En \\
PUBHEALTH~\citep{kotonya2020explainable} & Statement & 11,832  & Text & 4 Classes & Fact Check & En\\
COVID-Fact~\citep{SaakyanCM20} & Statement & 4,086  & Text & 2 Classes & Forum & En\\
X-Fact~\citep{gupta-srikumar-2021-x} & Statement & 31,189  & Text & 7 Classes & Fact Check & Many\\
\midrule
cQA~\citep{Mihaylova2018FactCI} & Answer & 422  & Meta & 2 Classes & Forum & En \\
% SemEval19-TB \citep{Mihaylova2019SemEval2019T8} & Answer & 917  & Meta & 3 & Forum & En \\
AnswerFact~\citep{Zhang2020AnswerFactFC} & Answer & 60,864 & Text & 5 Classes & Amazon & En \\
\midrule
% Hoax \citep{TacchiniBVMA17} & Article & 15,500  & Meta & 2 Classes & Facebook & En \\
NELA~\citep{HorneKA18} & Article & 136,000  & \xmark & 2 Classes & News & En \\
BuzzfeedNews \citep{Potthast2018ASI} & Article & 1,627 & Meta & 4 Classes & Facebook & En \\
BuzzFace~\citep{SantiaW18} & Article & 2,263 & Meta & 4 Classes & Facebook & En \\
% NELA18 \citep{Nrregaard2019NELAGT2018AL} & Article & 713,000 & 2 & \xmark & News & En \\
% NELA19 \citep{gruppi2020nela} & Article & 1.12M & 2 & \xmark & News & En \\
FA-KES~\citep{SalemFEJF19} & Article & 804 & \xmark & 2 Classes & VDC & En \\
FakeNewsNet \citep{Shu2018FakeNewsNetAD} & Article & 23,196  & Meta & 2 Classes & Fact Check & En \\
%FakeHealth \citep{DaiSW20} & Article & 2,296  & Meta & 2 Classes & Health & En \\
FakeCovid~\citep{shahifakecovid} & Article & 5,182  & \xmark & 2 Classes & Fact Check & Many \\
% \midrule
% Fauxtography \citep{Zlatkova2019FactCheckingMF} & Statement/Image & 1,233  & Meta & 2 & Fact Check/News & En \\
% Fakeddit \citep{Nakamura2020rFakedditAN} & Statement/Image & 1.06M  & Meta & 2,3,6 & Reddit & En \\
\bottomrule
\end{tabular}}
\vspace{-0.5em}
\caption{Summary of factual verification datasets with natural inputs. KG denotes knowledge graphs. ChectThat18 has been extended later~\citep{HasanainSEBN19,BarrnCedeo2020OverviewOC,NakovMEBMSAHHBN21}. NELA has been updated by adding more data from more diverse sources~\citep{NorregaardHA19,gruppi2020,gruppi2021} (Data collected by \cite{guo-etal-2022-survey})
}
\label{tab:natural}
\vspace{-1em}
\end{table*}
